Bose-Einstein Condensation of Atomic Hydrogen

This thesis describes the observation and study of Bose-Einstein condensation of a trapped, dilute gas of atomic hydrogen. The condensate and normal gas are studied by two-photon spectroscopy of the 1S-2S transition. We condense over 10^9 atoms per second for several seconds, and the peak condensate density is around 5x10^15 cm^-3. Topics covered in the thesis include a theoretical analysis of Bose-condensed hydrogen, a description of the cryogenic trapping cell and the evaporative cooling techniques used to bring the gas to the condensation point, and an analysis of the condensate.

==> forward.tex <==
%auto-ignore
% forward: my comments

This thesis is dedicated to Jesus Christ, who I understand to be the
One who created quantum mechanics, and indeed all of physics and the
whole of the entire universe.  The extremely rich and subtle
complexity of the physical world, and that of quantum systems such as
dilute gasses at low temperatures and high densities in particular,
give me reason to worship Him as an amazing intelligence with
creativity and complexity much farther beyond the grasp of the human
mind than the physics described in this thesis is beyond the grasp of
my sister-in-law's golden retriever.

Not only has the one who came to Earth as Jesus of Nazareth designed
and built the universe with all its beauty and intricacy and grandeur,
He has initiated a relationship with me that has implications vastly
beyond my activities here, or so He has informed me.  The
reconciliation and healing He has offered to me has allowed me to
pursue the studies described in this thesis.  This relationship gives
me even more reason to worship Him and give to Him my loyalty.  He is
the King of the Universe.

